Gaussian Process Regression and Classification using International Classification of Disease Codes as Covariates

International Classification of Disease (ICD) codes are widely used for encoding diagnoses in electronic health records (EHR). Automated methods have been developed over the years for predicting biomedical responses using EHR that borrow information among diagnostically similar patients. Relatively less attention has been paid to developing patient similarity measures that model the structure of ICD codes and the presence of multiple chronic conditions, where a chronic condition is defined as a set of ICD codes. Motivated by this problem, we first develop a type of string kernel function for measuring similarity between a pair of subsets of ICD codes, which uses the definition of chronic conditions. Second, we extend this similarity measure to define a family of covariance functions on subsets of ICD codes. Using this family, we develop Gaussian process (GP) priors for Bayesian nonparametric regression and classification using diagnoses and other demographic information as covariates. Markov chain Monte Carlo (MCMC) algorithms are used for posterior inference and predictions. The proposed methods are free of any tuning parameters and are well-suited for automated prediction of continuous and categorical biomedical responses that depend on chronic conditions. We evaluate the practical performance of our method on EHR data collected from 1660 patients at the University of Iowa Hospitals and Clinics (UIHC) with six different primary cancer sites. Our method has better sensitivity and specificity than its competitors in classifying different primary cancer sites and estimates the marginal associations between chronic conditions and primary cancer sites.

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
%\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}             %
\RequirePackage{amsbsy}             %
\RequirePackage{soul}

%%% MW %%%%

\newcommand{\mnote}[1]{{\bf\large *}\marginpar{\tiny#1}}
\newcommand{\dnote}[1]{{\bf\large +}\marginpar{\tiny#1}}
%\newcommand{\note}[1]{{\bf #1}}


%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

% \DeclareMathOperator{\ab}{\bmath{a}}
% \DeclareMathOperator{\bb}{\bmath{b}}
% \DeclareMathOperator{\cb}{\bmath{c}}
% \DeclareMathOperator{\db}{\bmath{d}}
% \DeclareMathOperator{\eb}{\bmath{e}}
% \DeclareMathOperator{\fb}{\bmath{f}}
% \DeclareMathOperator{\gb}{\bmath{g}}
% \DeclareMathOperator{\hb}{\bmath{h}}
% \DeclareMathOperator{\ib}{\bmath{i}}
% \DeclareMathOperator{\jb}{\bmath{j}}
% \DeclareMathOperator{\kb}{\bmath{k}}
% \DeclareMathOperator{\lb}{\bmath{l}}
% \DeclareMathOperator{\mb}{\bmath{m}}
% \DeclareMathOperator{\nbb}{\bmath{n}}
% \DeclareMathOperator{\ob}{\bmath{o}}
% \DeclareMathOperator{\pb}{\bmath{p}}
% \DeclareMathOperator{\qb}{\bmath{q}}
% \DeclareMathOperator{\rb}{\bmath{r}}
% \DeclareMathOperator{\sbb}{\bmath{s}}
% \DeclareMathOperator{\tb}{\bmath{t}}
% \DeclareMathOperator{\ub}{\bmath{u}}
% \DeclareMathOperator{\vb}{\bmath{v}}
% \DeclareMathOperator{\wb}{\bmath{w}}
% \DeclareMathOperator{\xb}{\bmath{x}}
% \DeclareMathOperator{\yb}{\bmath{y}}
% \DeclareMathOperator{\zb}{\bmath{z}}

\DeclareMathOperator{\ab}{\mathbf{a}}
\DeclareMathOperator{\bb}{\mathbf{b}}
\DeclareMathOperator{\cb}{\mathbf{c}}
\DeclareMathOperator{\db}{\mathbf{d}}
\DeclareMathOperator{\eb}{\mathbf{e}}
\DeclareMathOperator{\fb}{\mathbf{f}}
\DeclareMathOperator{\gb}{\mathbf{g}}
\DeclareMathOperator{\hb}{\mathbf{h}}
\DeclareMathOperator{\ib}{\mathbf{i}}
\DeclareMathOperator{\jb}{\mathbf{j}}
\DeclareMathOperator{\kb}{\mathbf{k}}
\DeclareMathOperator{\lb}{\mathbf{l}}
\DeclareMathOperator{\mb}{\mathbf{m}}
\DeclareMathOperator{\nbb}{\mathbf{n}}
\DeclareMathOperator{\ob}{\mathbf{o}}
\DeclareMathOperator{\pb}{\mathbf{p}}
\DeclareMathOperator{\qb}{\mathbf{q}}
\DeclareMathOperator{\rb}{\mathbf{r}}
\DeclareMathOperator{\sbb}{\mathbf{s}}
\DeclareMathOperator{\tb}{\mathbf{t}}
\DeclareMathOperator{\ub}{\mathbf{u}}
\DeclareMathOperator{\vb}{\mathbf{v}}
\DeclareMathOperator{\wb}{\mathbf{w}}
\DeclareMathOperator{\xb}{\mathbf{x}}
\DeclareMathOperator{\yb}{\mathbf{y}}
\DeclareMathOperator{\zb}{\mathbf{z}}

\DeclareMathOperator{\atilde}{\tilde{\ab}}
\DeclareMathOperator{\btilde}{\tilde{\bb}}
\DeclareMathOperator{\ctilde}{\tilde{\cb}}
\DeclareMathOperator{\dtilde}{\tilde{\db}}
\DeclareMathOperator{\etilde}{\tilde{\eb}}
\DeclareMathOperator{\ftilde}{\tilde{\fb}}
\DeclareMathOperator{\gtilde}{\tilde{\gb}}
\DeclareMathOperator{\htilde}{\tilde{\hb}}
\DeclareMathOperator{\itilde}{\tilde{\ib}}
\DeclareMathOperator{\jtilde}{\tilde{\jb}}
\DeclareMathOperator{\ktilde}{\tilde{\kb}}
\DeclareMathOperator{\ltilde}{\tilde{\lb}}
\DeclareMathOperator{\mtilde}{\tilde{\mb}}
\DeclareMathOperator{\ntilde}{\tilde{\nbb}}
\DeclareMathOperator{\otilde}{\tilde{\ob}}
%
\DeclareMathOperator{\qtilde}{\tilde{\qb}}
\DeclareMathOperator{\rtilde}{\tilde{\rb}}
\DeclareMathOperator{\stilde}{\tilde{\sbb}}
\DeclareMathOperator{\ttilde}{\tilde{\tb}}
\DeclareMathOperator{\utilde}{\tilde{\ub}}
\DeclareMathOperator{\vtilde}{\tilde{\vb}}
\DeclareMathOperator{\wtilde}{\tilde{\wb}}
\DeclareMathOperator{\xtilde}{\tilde{\xb}}
\DeclareMathOperator{\ytilde}{\tilde{\yb}}
\DeclareMathOperator{\ztilde}{\tilde{\zb}}

\DeclareMathOperator{\thetabar}{\overline{\theta}}
\DeclareMathOperator{\abar}{\overline{a}}
\DeclareMathOperator{\bbar}{\overline{b}}
\DeclareMathOperator{\cbar}{\overline{c}}
\DeclareMathOperator{\dbar}{\overline{d}}
\DeclareMathOperator{\ebar}{\overline{e}}
\DeclareMathOperator{\fbar}{\overline{f}}
\DeclareMathOperator{\gbar}{\overline{g}}
\DeclareMathOperator{\hbbar}{\overline{h}}
\DeclareMathOperator{\ibar}{\overline{i}}
\DeclareMathOperator{\jbar}{\overline{j}}
\DeclareMathOperator{\kbar}{\overline{k}}
\DeclareMathOperator{\lbar}{\overline{l}}
\DeclareMathOperator{\mbar}{\overline{m}}
\DeclareMathOperator{\nbar}{\overline{n}}
\DeclareMathOperator{\obar}{\overline{o}}
\DeclareMathOperator{\pbar}{\overline{p}}
\DeclareMathOperator{\qbar}{\overline{q}}
\DeclareMathOperator{\rbar}{\overline{r}}
\DeclareMathOperator{\sbar}{\overline{s}}
\DeclareMathOperator{\tbar}{\overline{t}}
\DeclareMathOperator{\ubar}{\overline{u}}
\DeclareMathOperator{\vbar}{\overline{v}}
\DeclareMathOperator{\wbar}{\overline{w}}
\DeclareMathOperator{\xbar}{\overline{x}}
\DeclareMathOperator{\ybar}{\overline{y}}
\DeclareMathOperator{\zbar}{\overline{z}}

% \DeclareMathOperator{\Ab}{\bmath{A}}
% \DeclareMathOperator{\Bb}{\bmath{B}}
% \DeclareMathOperator{\Cb}{\bmath{C}}
% \DeclareMathOperator{\Db}{\bmath{D}}
% \DeclareMathOperator{\Eb}{\bmath{E}}
% \DeclareMathOperator{\Gb}{\bmath{G}}
% \DeclareMathOperator{\Hb}{\bmath{H}}
% \DeclareMathOperator{\Ib}{\bmath{I}}
% \DeclareMathOperator{\Jb}{\bmath{J}}
% \DeclareMathOperator{\Kb}{\bmath{K}}
% \DeclareMathOperator{\Lb}{\bmath{L}}
% \DeclareMathOperator{\Mb}{\bmath{M}}
% \DeclareMathOperator{\Nb}{\bmath{N}}
% \DeclareMathOperator{\Ob}{\bmath{O}}
% \DeclareMathOperator{\Pb}{\bmath{P}}
% \DeclareMathOperator{\Qb}{\bmath{Q}}
% \DeclareMathOperator{\Rb}{\bmath{R}}
% \DeclareMathOperator{\Sbb}{\bmath{S}}
% \DeclareMathOperator{\Tb}{\bmath{T}}
% \DeclareMathOperator{\Ub}{\bmath{U}}
% \DeclareMathOperator{\Vb}{\bmath{V}}
% \DeclareMathOperator{\Wb}{\bmath{W}}
% \DeclareMathOperator{\Xb}{\bmath{X}}
% \DeclareMathOperator{\Yb}{\bmath{Y}}
% \DeclareMathOperator{\Zb}{\bmath{Z}}

\DeclareMathOperator{\Ab}{\mathbf{A}}
\DeclareMathOperator{\Bb}{\mathbf{B}}
\DeclareMathOperator{\Cb}{\mathbf{C}}
\DeclareMathOperator{\Db}{\mathbf{D}}
\DeclareMathOperator{\Eb}{\mathbf{E}}
\DeclareMathOperator{\Fb}{\mathbf{F}}
\DeclareMathOperator{\Gb}{\mathbf{G}}
\DeclareMathOperator{\Hb}{\mathbf{H}}
\DeclareMathOperator{\Ib}{\mathbf{I}}
\DeclareMathOperator{\Jb}{\mathbf{J}}
\DeclareMathOperator{\Kb}{\mathbf{K}}
\DeclareMathOperator{\Lb}{\mathbf{L}}
\DeclareMathOperator{\Mb}{\mathbf{M}}
\DeclareMathOperator{\Nb}{\mathbf{N}}
\DeclareMathOperator{\Ob}{\mathbf{O}}
\DeclareMathOperator{\Pb}{\mathbf{P}}
\DeclareMathOperator{\Qb}{\mathbf{Q}}
\DeclareMathOperator{\Rb}{\mathbf{R}}
\DeclareMathOperator{\Sbb}{\mathbf{S}}
\DeclareMathOperator{\Tb}{\mathbf{T}}
\DeclareMathOperator{\Ub}{\mathbf{U}}
\DeclareMathOperator{\Vb}{\mathbf{V}}
\DeclareMathOperator{\Wb}{\mathbf{W}}
\DeclareMathOperator{\Xb}{\mathbf{X}}
\DeclareMathOperator{\Yb}{\mathbf{Y}}
\DeclareMathOperator{\Zb}{\mathbf{Z}}
\DeclareMathOperator{\Abar}{\bar{A}}
\DeclareMathOperator{\Bbar}{\bar{B}}
\DeclareMathOperator{\Cbar}{\bar{C}}
\DeclareMathOperator{\Dbar}{\bar{D}}
\DeclareMathOperator{\Ebar}{\bar{E}}
\DeclareMathOperator{\Fbar}{\bar{F}}
\DeclareMathOperator{\Gbar}{\bar{G}}
\DeclareMathOperator{\Hbar}{\bar{H}}
\DeclareMathOperator{\Ibar}{\bar{I}}
\DeclareMathOperator{\Jbar}{\bar{J}}
\DeclareMathOperator{\Kbar}{\bar{K}}
\DeclareMathOperator{\Lbar}{\bar{L}}
\DeclareMathOperator{\Mbar}{\bar{M}}
\DeclareMathOperator{\Nbar}{\bar{N}}
\DeclareMathOperator{\Obar}{\bar{O}}
\DeclareMathOperator{\Pbar}{\bar{P}}
\DeclareMathOperator{\Qbar}{\bar{Q}}
\DeclareMathOperator{\Rbar}{\bar{R}}
\DeclareMathOperator{\Sbar}{\bar{S}}
\DeclareMathOperator{\Tbar}{\bar{T}}
\DeclareMathOperator{\Ubar}{\bar{U}}
\DeclareMathOperator{\Vbar}{\bar{V}}
\DeclareMathOperator{\Wbar}{\bar{W}}
\DeclareMathOperator{\Xbar}{\bar{X}}
\DeclareMathOperator{\Ybar}{\bar{Y}}
\DeclareMathOperator{\Zbar}{\bar{Z}}

\DeclareMathOperator{\Abbar}{\overline{\Ab}}
\DeclareMathOperator{\Bbbar}{\overline{\Bb}}
\DeclareMathOperator{\Cbbar}{\overline{\Cb}}
\DeclareMathOperator{\Dbbar}{\overline{\Db}}
\DeclareMathOperator{\Ebbar}{\overline{\Eb}}
\DeclareMathOperator{\Fbbar}{\overline{\Fb}}
\DeclareMathOperator{\Gbbar}{\overline{\Gb}}
\DeclareMathOperator{\Hbbar}{\overline{\Hb}}
\DeclareMathOperator{\Ibbar}{\overline{\Ib}}
\DeclareMathOperator{\Jbbar}{\overline{\Jb}}
\DeclareMathOperator{\Kbbar}{\overline{\Kb}}
\DeclareMathOperator{\Lbbar}{\overline{\Lb}}
\DeclareMathOperator{\Mbbar}{\overline{\Mb}}
\DeclareMathOperator{\Nbbar}{\overline{\Nb}}
\DeclareMathOperator{\Obbar}{\overline{\Ob}}
\DeclareMathOperator{\Pbbar}{\overline{\Pb}}
\DeclareMathOperator{\Qbbar}{\overline{\Qb}}
\DeclareMathOperator{\Rbbar}{\overline{\Rb}}
\DeclareMathOperator{\Sbbar}{\overline{\Sb}}
\DeclareMathOperator{\Tbbar}{\overline{\Tb}}
\DeclareMathOperator{\Ubbar}{\overline{\Ub}}
\DeclareMathOperator{\Vbbar}{\overline{\Vb}}
\DeclareMathOperator{\Wbbar}{\overline{\Wb}}
\DeclareMathOperator{\Xbbar}{\overline{\Xb}}
\DeclareMathOperator{\Ybbar}{\overline{\Yb}}
\DeclareMathOperator{\Zbbar}{\overline{\Zb}}

\DeclareMathOperator{\Ahat}{\widehat{A}}
\DeclareMathOperator{\Bhat}{\widehat{B}}
\DeclareMathOperator{\Chat}{\widehat{C}}
\DeclareMathOperator{\Dhat}{\widehat{D}}
\DeclareMathOperator{\Ehat}{\widehat{E}}
\DeclareMathOperator{\Fhat}{\widehat{F}}
\DeclareMathOperator{\Ghat}{\widehat{G}}
\DeclareMathOperator{\Hhat}{\widehat{H}}
\DeclareMathOperator{\Ihat}{\widehat{I}}
\DeclareMathOperator{\Jhat}{\widehat{J}}
\DeclareMathOperator{\Khat}{\widehat{K}}
\DeclareMathOperator{\Lhat}{\widehat{L}}
\DeclareMathOperator{\Mhat}{\widehat{M}}
\DeclareMathOperator{\Nhat}{\widehat{N}}
\DeclareMathOperator{\Ohat}{\widehat{O}}
\DeclareMathOperator{\Phat}{\widehat{P}}
\DeclareMathOperator{\Qhat}{\widehat{Q}}
\DeclareMathOperator{\Rhat}{\widehat{R}}
\DeclareMathOperator{\Shat}{\widehat{S}}
\DeclareMathOperator{\That}{\widehat{T}}
\DeclareMathOperator{\Uhat}{\widehat{U}}
\DeclareMathOperator{\Vhat}{\widehat{V}}
\DeclareMathOperator{\What}{\widehat{W}}
\DeclareMathOperator{\Xhat}{\widehat{X}}
\DeclareMathOperator{\Yhat}{\widehat{Y}}
\DeclareMathOperator{\Zhat}{\widehat{Z}}

\DeclareMathOperator{\Abhat}{\widehat{\Ab}}
\DeclareMathOperator{\Bbhat}{\widehat{\Bb}}
\DeclareMathOperator{\Cbhat}{\widehat{\Cb}}
\DeclareMathOperator{\Dbhat}{\widehat{\Db}}
\DeclareMathOperator{\Ebhat}{\widehat{\Eb}}
\DeclareMathOperator{\Fbhat}{\widehat{\Fb}}
\DeclareMathOperator{\Gbhat}{\widehat{\Gb}}
\DeclareMathOperator{\Hbhat}{\widehat{\Hb}}
\DeclareMathOperator{\Ibhat}{\widehat{\Ib}}
\DeclareMathOperator{\Jbhat}{\widehat{\Jb}}
\DeclareMathOperator{\Kbhat}{\widehat{\Kb}}
\DeclareMathOperator{\Lbhat}{\widehat{\Lb}}
\DeclareMathOperator{\Mbhat}{\widehat{\Mb}}
\DeclareMathOperator{\Nbhat}{\widehat{\Nb}}
\DeclareMathOperator{\Obhat}{\widehat{\Ob}}
\DeclareMathOperator{\Pbhat}{\widehat{\Pb}}
\DeclareMathOperator{\Qbhat}{\widehat{\Qb}}
\DeclareMathOperator{\Rbhat}{\widehat{\Rb}}
\DeclareMathOperator{\Sbhat}{\widehat{\Sb}}
\DeclareMathOperator{\Tbhat}{\widehat{\Tb}}
\DeclareMathOperator{\Ubhat}{\widehat{\Ub}}
\DeclareMathOperator{\Vbhat}{\widehat{\Vb}}
\DeclareMathOperator{\Wbhat}{\widehat{\Wb}}
\DeclareMathOperator{\Xbhat}{\widehat{\Xb}}
\DeclareMathOperator{\Ybhat}{\widehat{\Yb}}
\DeclareMathOperator{\Zbhat}{\widehat{\Zb}}

\DeclareMathOperator{\Acal}{\mathcal{A}}
\DeclareMathOperator{\Bcal}{\mathcal{B}}
\DeclareMathOperator{\Ccal}{\mathcal{C}}
\DeclareMathOperator{\Dcal}{\mathcal{D}}
\DeclareMathOperator{\Ecal}{\mathcal{E}}
\DeclareMathOperator{\Fcal}{\mathcal{F}}
\DeclareMathOperator{\Gcal}{\mathcal{G}}
\DeclareMathOperator{\Hcal}{\mathcal{H}}
\DeclareMathOperator{\Ical}{\mathcal{I}}
\DeclareMathOperator{\Jcal}{\mathcal{J}}
\DeclareMathOperator{\Kcal}{\mathcal{K}}
\DeclareMathOperator{\Lcal}{\mathcal{L}}
\DeclareMathOperator{\Mcal}{\mathcal{M}}
\DeclareMathOperator{\Ncal}{\mathcal{N}}
\DeclareMathOperator{\Ocal}{\mathcal{O}}
\DeclareMathOperator{\Pcal}{\mathcal{P}}
\DeclareMathOperator{\Qcal}{\mathcal{Q}}
\DeclareMathOperator{\Rcal}{\mathcal{R}}
\DeclareMathOperator{\Scal}{\mathcal{S}}
\DeclareMathOperator{\Tcal}{\mathcal{T}}
\DeclareMathOperator{\Ucal}{\mathcal{U}}
\DeclareMathOperator{\Vcal}{\mathcal{V}}
\DeclareMathOperator{\Wcal}{\mathcal{W}}
\DeclareMathOperator{\Xcal}{\mathcal{X}}
\DeclareMathOperator{\Ycal}{\mathcal{Y}}
\DeclareMathOperator{\Zcal}{\mathcal{Z}}

\DeclareMathOperator{\Afrak}{\mathfrak{A}}
\DeclareMathOperator{\Bfrak}{\mathfrak{B}}
\DeclareMathOperator{\Cfrak}{\mathfrak{C}}
\DeclareMathOperator{\Dfrak}{\mathfrak{D}}
\DeclareMathOperator{\Efrak}{\mathfrak{E}}
\DeclareMathOperator{\Ffrak}{\mathfrak{F}}
\DeclareMathOperator{\Gfrak}{\mathfrak{G}}
\DeclareMathOperator{\Hfrak}{\mathfrak{H}}
\DeclareMathOperator{\Ifrak}{\mathfrak{I}}
\DeclareMathOperator{\Jfrak}{\mathfrak{J}}
\DeclareMathOperator{\Kfrak}{\mathfrak{K}}
\DeclareMathOperator{\Lfrak}{\mathfrak{L}}
\DeclareMathOperator{\Mfrak}{\mathfrak{M}}
\DeclareMathOperator{\Nfrak}{\mathfrak{N}}
\DeclareMathOperator{\Ofrak}{\mathfrak{O}}
\DeclareMathOperator{\Pfrak}{\mathfrak{P}}
\DeclareMathOperator{\Qfrak}{\mathfrak{Q}}
\DeclareMathOperator{\Rfrak}{\mathfrak{R}}
\DeclareMathOperator{\Sfrak}{\mathfrak{S}}
\DeclareMathOperator{\Tfrak}{\mathfrak{T}}
\DeclareMathOperator{\Ufrak}{\mathfrak{U}}
\DeclareMathOperator{\Vfrak}{\mathfrak{V}}
\DeclareMathOperator{\Wfrak}{\mathfrak{W}}
\DeclareMathOperator{\Xfrak}{\mathfrak{X}}
\DeclareMathOperator{\Yfrak}{\mathfrak{Y}}
\DeclareMathOperator{\Zfrak}{\mathfrak{Z}}

\DeclareMathOperator{\Ascr}{\mathscr{A}}
\DeclareMathOperator{\Bscr}{\mathscr{B}}
\DeclareMathOperator{\Cscr}{\mathscr{C}}
\DeclareMathOperator{\Dscr}{\mathscr{D}}
\DeclareMathOperator{\Escr}{\mathscr{E}}
\DeclareMathOperator{\Fscr}{\mathscr{F}}
\DeclareMathOperator{\Gscr}{\mathscr{G}}
\DeclareMathOperator{\Hscr}{\mathscr{H}}
\DeclareMathOperator{\Iscr}{\mathscr{I}}
\DeclareMathOperator{\Jscr}{\mathscr{J}}
\DeclareMathOperator{\Kscr}{\mathscr{K}}
\DeclareMathOperator{\Lscr}{\mathscr{L}}
\DeclareMathOperator{\Mscr}{\mathscr{M}}
\DeclareMathOperator{\Nscr}{\mathscr{N}}
\DeclareMathOperator{\Oscr}{\mathscr{O}}
\DeclareMathOperator{\Pscr}{\mathscr{P}}
\DeclareMathOperator{\Qscr}{\mathscr{Q}}
\DeclareMathOperator{\Rscr}{\mathscr{R}}
\DeclareMathOperator{\Sscr}{\mathscr{S}}
\DeclareMathOperator{\Tscr}{\mathscr{T}}
\DeclareMathOperator{\Uscr}{\mathscr{U}}
\DeclareMathOperator{\Vscr}{\mathscr{V}}
\DeclareMathOperator{\Wscr}{\mathscr{W}}
\DeclareMathOperator{\Xscr}{\mathscr{X}}
\DeclareMathOperator{\Yscr}{\mathscr{Y}}
\DeclareMathOperator{\Zscr}{\mathscr{Z}}

\DeclareMathOperator{\Atilde}{\widetilde{A}}
\DeclareMathOperator{\Btilde}{\widetilde{B}}
\DeclareMathOperator{\Ctilde}{\widetilde{C}}
\DeclareMathOperator{\Dtilde}{\widetilde{D}}
\DeclareMathOperator{\Etilde}{\widetilde{E}}
\DeclareMathOperator{\Ftilde}{\widetilde{F}}
\DeclareMathOperator{\Gtilde}{\widetilde{G}}
\DeclareMathOperator{\Htilde}{\widetilde{H}}
\DeclareMathOperator{\Itilde}{\widetilde{I}}
\DeclareMathOperator{\Jtilde}{\widetilde{J}}
\DeclareMathOperator{\Ktilde}{\widetilde{K}}
\DeclareMathOperator{\Ltilde}{\widetilde{L}}
\DeclareMathOperator{\Mtilde}{\widetilde{M}}
\DeclareMathOperator{\Ntilde}{\widetilde{N}}
\DeclareMathOperator{\Otilde}{\widetilde{O}}
\DeclareMathOperator{\Ptilde}{\widetilde{P}}
\DeclareMathOperator{\Qtilde}{\widetilde{Q}}
\DeclareMathOperator{\Rtilde}{\widetilde{R}}
\DeclareMathOperator{\Stilde}{\widetilde{S}}
\DeclareMathOperator{\Ttilde}{\widetilde{T}}
\DeclareMathOperator{\Utilde}{\widetilde{U}}
\DeclareMathOperator{\Vtilde}{\widetilde{V}}
\DeclareMathOperator{\Wtilde}{\widetilde{W}}
\DeclareMathOperator{\Xtilde}{\widetilde{X}}
\DeclareMathOperator{\Ytilde}{\widetilde{Y}}
\DeclareMathOperator{\Ztilde}{\widetilde{Z}}


%%%%%%%% Widely accepted definitions %%%%%%%%%%%%%%%

\DeclareMathOperator{\CC}{\mathbb{C}} % Complex numbers
\DeclareMathOperator{\EE}{\mathbb{E}} % Expectation
\DeclareMathOperator{\KK}{\mathbb{K}} % Arbitrary field
\DeclareMathOperator{\MM}{\mathbb{M}} % Median
\DeclareMathOperator{\NN}{\mathbb{N}} % Natural numbers
\DeclareMathOperator{\PP}{\mathbb{P}} % Probability
\DeclareMathOperator{\QQ}{\mathbb{Q}} % Rationals
\DeclareMathOperator{\RR}{\mathbb{R}} % Real numbers
\DeclareMathOperator{\ZZ}{\mathbb{Z}} % Integers
\DeclareMathOperator{\II}{\mathbb{I}}
\DeclareMathOperator{\VV}{\mathbb{V}}
\DeclareMathOperator{\BB}{\mathbb{B}}
\DeclareMathOperator{\HH}{\mathbb{H}}
\DeclareMathOperator{\LL}{\mathbb{L}}

\DeclareMathOperator{\one}{\mathbf{1}}  % Identity
\DeclareMathOperator{\zero}{\mathbf{0}} % Zero

\DeclareMathOperator*{\mini}{\mathop{\mathrm{minimize}}}
\DeclareMathOperator*{\maxi}{\mathop{\mathrm{maximize}}}

\DeclareMathOperator{\sgn}{\mathop{\mathrm{sign}}}
\DeclareMathOperator{\rank}{\mathop{\mathrm{rank}}}
\DeclareMathOperator{\traj}{\mathop{\mathrm{Traj}}}

%%%%%%%% Bold Greek Letters %%%%%%%%%%%%%%%
% \DeclareMathOperator{\alphab}{{\bmath{\alpha}}}
% \DeclareMathOperator{\betab}{{\bmath{\beta}}}
% \DeclareMathOperator{\gammab}{{\bmath{\gamma}}}
% \DeclareMathOperator{\deltab}{{\bmath{\delta}}}
% \DeclareMathOperator{\epsilonb}{{\bmath{\epsilon}}}
% \DeclareMathOperator{\varepsilonb}{{\bmath{\varepsilon}}}
% \DeclareMathOperator{\zetab}{{\bmath{\zeta}}}
% \DeclareMathOperator{\etab}{{\bmath{\eta}}}
% \DeclareMathOperator{\thetab}{{\bmath{\theta}}}
% \DeclareMathOperator{\varthetab}{{\bmath{\vartheta}}}
% \DeclareMathOperator{\kappab}{{\bmath{\kappa}}}
% \DeclareMathOperator{\lambdab}{{\bmath{\lambda}}}
% \DeclareMathOperator{\mub}{{\bmath{\mu}}}
% \DeclareMathOperator{\nub}{{\bmath{\nu}}}
% \DeclareMathOperator{\xib}{{\bmath{\xi}}}
% \DeclareMathOperator{\pib}{{\bmath{\pi}}}
% \DeclareMathOperator{\varpib}{{\bmath{\varpi}}}
% \DeclareMathOperator{\rhob}{{\bmath{\rho}}}
% \DeclareMathOperator{\varrhob}{{\bmath{\varrho}}}
% \DeclareMathOperator{\sigmab}{{\bmath{\sigma}}}
% \DeclareMathOperator{\varsigmab}{{\bmath{\varsigma}}}
% \DeclareMathOperator{\taub}{{\bmath{\tau}}}
% \DeclareMathOperator{\upsilonb}{{\bmath{\upsilon}}}
% \DeclareMathOperator{\phib}{{\bmath{\phi}}}
% \DeclareMathOperator{\varphib}{{\bmath{\varphi}}}
% \DeclareMathOperator{\chib}{{\bmath{\chi}}}
% \DeclareMathOperator{\psib}{{\bmath{\psi}}}
% \DeclareMathOperator{\omegab}{{\bmath{\omega}}}
% \DeclareMathOperator{\Gammab}{{\bmath{\Gamma}}}
% \DeclareMathOperator{\Deltab}{{\bmath{\Delta}}}
% \DeclareMathOperator{\Thetab}{{\bmath{\Theta}}}
% \DeclareMathOperator{\Lambdab}{{\bmath{\Lambda}}}
% \DeclareMathOperator{\Xib}{{\bmath{\Xi}}}
% \DeclareMathOperator{\Pib}{{\bmath{\Pi}}}
% \DeclareMathOperator{\Sigmab}{{\bmath{\Sigma}}}
% \DeclareMathOperator{\Upsilonb}{{\bmath{\Upsilon}}}
% \DeclareMathOperator{\Phib}{{\bmath{\Phi}}}
% \DeclareMathOperator{\Psib}{{\bmath{\Psi}}}
% \DeclareMathOperator{\Omegab}{{\bmath{\Omega}}}

\DeclareMathOperator{\alphab}{{\mathbf{\alpha}}}
\DeclareMathOperator{\betab}{{\mathbf{\beta}}}
\DeclareMathOperator{\gammab}{{\mathbf{\gamma}}}
\DeclareMathOperator{\deltab}{{\mathbf{\delta}}}
\DeclareMathOperator{\epsilonb}{{\mathbf{\epsilon}}}
\DeclareMathOperator{\varepsilonb}{{\mathbf{\varepsilon}}}
\DeclareMathOperator{\zetab}{{\mathbf{\zeta}}}
\DeclareMathOperator{\etab}{{\mathbf{\eta}}}
\DeclareMathOperator{\thetab}{{\mathbf{\theta}}}
\DeclareMathOperator{\varthetab}{{\mathbf{\vartheta}}}
\DeclareMathOperator{\kappab}{{\mathbf{\kappa}}}
\DeclareMathOperator{\lambdab}{{\mathbf{\lambda}}}
\DeclareMathOperator{\mub}{{\mathbf{\mu}}}
\DeclareMathOperator{\nub}{{\mathbf{\nu}}}
\DeclareMathOperator{\xib}{{\mathbf{\xi}}}
\DeclareMathOperator{\pib}{{\mathbf{\pi}}}
\DeclareMathOperator{\varpib}{{\mathbf{\varpi}}}
\DeclareMathOperator{\rhob}{{\mathbf{\rho}}}
\DeclareMathOperator{\varrhob}{{\mathbf{\varrho}}}
\DeclareMathOperator{\sigmab}{{\mathbf{\sigma}}}
\DeclareMathOperator{\varsigmab}{{\mathbf{\varsigma}}}
\DeclareMathOperator{\taub}{{\mathbf{\tau}}}
\DeclareMathOperator{\upsilonb}{{\mathbf{\upsilon}}}
\DeclareMathOperator{\phib}{{\mathbf{\phi}}}
\DeclareMathOperator{\varphib}{{\mathbf{\varphi}}}
\DeclareMathOperator{\chib}{{\mathbf{\chi}}}
\DeclareMathOperator{\psib}{{\mathbf{\psi}}}
\DeclareMathOperator{\omegab}{{\mathbf{\omega}}}
\DeclareMathOperator{\Gammab}{{\mathbf{\Gamma}}}
\DeclareMathOperator{\Deltab}{{\mathbf{\Delta}}}
\DeclareMathOperator{\Thetab}{{\mathbf{\Theta}}}
\DeclareMathOperator{\Lambdab}{{\mathbf{\Lambda}}}
\DeclareMathOperator{\Xib}{{\mathbf{\Xi}}}
\DeclareMathOperator{\Pib}{{\mathbf{\Pi}}}
\DeclareMathOperator{\Sigmab}{{\mathbf{\Sigma}}}
\DeclareMathOperator{\Upsilonb}{{\mathbf{\Upsilon}}}
\DeclareMathOperator{\Phib}{{\mathbf{\Phi}}}
\DeclareMathOperator{\Psib}{{\mathbf{\Psi}}}
\DeclareMathOperator{\Omegab}{{\mathbf{\Omega}}}

\DeclareMathOperator{\Gammacal}{{\mathcal{\Gamma}}}
\DeclareMathOperator{\Deltacal}{{\mathcal{\Delta}}}
\DeclareMathOperator{\Thetacal}{{\mathcal{\Theta}}}
\DeclareMathOperator{\Lambdacal}{{\mathcal{\Lambda}}}
\DeclareMathOperator{\Xical}{{\mathcal{\Xi}}}
\DeclareMathOperator{\Pical}{{\mathcal{\Pi}}}
\DeclareMathOperator{\Sigmacal}{{\mathcal{\Sigma}}}
\DeclareMathOperator{\Upsiloncal}{{\mathcal{\Upsilon}}}
\DeclareMathOperator{\Phical}{{\mathcal{\Phi}}}
\DeclareMathOperator{\Psical}{{\mathcal{\Psi}}}
\DeclareMathOperator{\Omegacal}{{\mathcal{\Omega}}}

%%%%%%%% Mess around with LaTeX %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem{assumption}[theorem]{Assumption}

\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{question}[theorem]{Question}

%\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
%\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

% % \ifx\theorem\undefined
% % \newtheorem{theorem}{Theorem}
% % \fi
% \ifx\example\undefined
% \newtheorem{example}{Example}
% \fi
% % \ifx\lemma\undefined
% % \newtheorem{lemma}[theorem]{Lemma}
% % \fi

% \ifx\corollary\undefined
% \newtheorem{corollary}[theorem]{Corollary}
% \fi

% \ifx\definition\undefined
% \newtheorem{definition}[theorem]{Definition}
% \fi

% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{conjecture}[theorem]{Conjecture}

% \newtheorem{factoid}[theorem]{Fact}


%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}

\newcommand{\ea}{\emph{et al. }}
\newcommand{\eg}{\emph{e.g. }}
\newcommand{\ie}{\emph{i.e., }}

\newcommand{\sri}[1]{\textcolor{red}{{\slshape #1}}}

%Logic
%\newcommand{\implies}{\Rightarrow}
%\newcommand{\iff}{\Leftrightarrow}
\newcommand{\goesto}{\longrightarrow}
\newcommand{\suchthat}{\ensuremathmode{\text{ such that }}}
%\newcommand{\st}{\suchthat}

%%%%%%%% Specific symbols for this project %%%%%%%%%%%%%%%

% upright names for matrices --don't use for single-letter function names!
\DeclareMathOperator{\DD}{\mathbb{D}} % DD
\DeclareMathOperator{\Thetabb}{\mathcal{C}} % DD

\DeclareMathOperator{\dd}{\mathrm{d}}

% Dual Spaces
\DeclareMathOperator{\Xcals}{\Xcal^{*}}
\DeclareMathOperator{\Mcals}{\Mcal^{*}}

% set and domain concepts
\DeclareMathOperator{\ri}{\mathrm{ri}}      % Relative interior
\DeclareMathOperator{\intr}{\mathrm{int}}   % Interior
\DeclareMathOperator{\bd}{\mathrm{bdry}}      % Boundary (see RocWet98)
\DeclareMathOperator{\dom}{\mathrm{dom}}    % Effective Domain
\DeclareMathOperator{\epi}{\mathrm{epi}}    % Epigraph
\DeclareMathOperator{\ran}{\mathrm{range}}  % Range of an operator

\newcommand{\by}{\times}

% gradient: \grad{F}{\m}
\newcommand{\grad}[2]{\nabla #1 \left( #2 \right) }
\newcommand{\hess}[2]{\nabla^2 #1 \left( #2 \right) }
\newcommand{\grd}{\nabla} % simpler version!
\newcommand{\breg}[1]{\Delta #1} % Bregman divergence

% subgradient: \subgrad{F}{\m}
\newcommand{\subgrad}[2]{\partial #1 \left( #2 \right) }
% subdiferential
\newcommand{\subdiff}{\partial}

% Vector of all ones
\newcommand{\ones}{\eb}

% Sum from i equal 1 to n
\newcommand{\sumin}{\sum_{i=1}^{n}}
\newcommand{\sumjn}{\sum_{j=1}^{n}}

% Deformed logarithm wrt \phi
\newcommand{\lphi}{\log_{\phi}}

% function k_{\phi}
\newcommand{\kphi}{k_{\phi}}

% reparam for dual log
\newcommand{\phibl}{\phi^{\bullet}}
\newcommand{\psibl}{\psi^{\bullet}}

% Deformed exponential wrt \phi
\newcommand{\ephi}{\exp_{\phi}}

% One over deformed exponential wrt \phi
\newcommand{\ephibl}{\exp^{\bullet}_{\phi}}

% Gradient of deformed exponential wrt \phi
\newcommand{\ephip}{\nabla_{x} \exp_{\phi}}

% Gradient of t-exponential wrt \phi
\newcommand{\ephit}{\nabla_{x} \exp_{t}}

% Deformed logarithm wrt \psi
\newcommand{\lpsi}{\log_{\psi}}

% One over deformed logarithm wrt \psi
\newcommand{\lpsib}{\log^{\bullet}_{\psi}}
\newcommand{\lphibl}{\log^{\bullet}_{\phi}}

%composition needed for conjugate--formerly combo
\newcommand{\lcirce}{\lpsi \circ \ephibl}

% S and related
\newcommand{\Sp}{S_{\phi}}
\newcommand{\Sps}{S^{*}_{\phi}}
\newcommand{\smp}{s_{\phi}}
\newcommand{\smpp}{s^{\prime}_{\phi}}
\newcommand{\smps}{s^{*}_{\phi}}

% T
\DeclareMathOperator{\tp}{\tilde{p}}
\newcommand{\tgamma}{\tilde{\gamma}}
\newcommand{\tGamma}{\tilde{\Gamma}}
\DeclareMathOperator{\tq}{\tilde{q}}
\DeclareMathOperator{\tg}{\tilde{g}}
\DeclareMathOperator{\tmu}{\tilde{\mu}}
\DeclareMathOperator{\tthe}{\tilde{\theta}}
\DeclareMathOperator{\ttheb}{\tilde{\bm{\theta}}}
\DeclareMathOperator{\tmc}{\widehat{\Mcal}}
\DeclareMathOperator{\tv}{\tilde{v}}

\DeclareMathOperator{\Remp}{R_{\text{emp}}}

